Trace Abstraction Modulo Probability

We propose trace abstraction modulo probability, a proof technique for verifying high-probability accuracy guarantees of probabilistic programs. Our proofs overapproximate the set of program traces using failure automata, finite-state automata that upper bound the probability of failing to satisfy a target specification. We automate proof construction by reducing probabilistic reasoning to logical reasoning: we use program synthesis methods to select axioms for sampling instructions, and then apply Craig interpolation to prove that traces fail the target specification with only a small probability. Our method handles programs with unknown inputs, parameterized distributions, infinite state spaces, and parameterized specifications. We evaluate our technique on a range of randomized algorithms drawn from the differential privacy literature and beyond. To our knowledge, our approach is the first to automatically establish accuracy properties of these algorithms.

==> discussion.tex <==
\paragraph{Pre-Expectation Calculus}The pre-expectation calculus and associated predicate transformers \citep{Kozen:1985, Morgan:1996} can prove properties of probabilistic programs, but introduces significant practical challenges towards full automation. Computing pre-expectations across sampling instructions yields an integral over the distribution being sampled from. Complex distributions, like the infinite-support Laplace distribution common in differential privacy, yield correspondingly complex integrals that are difficult to reason about. Any automation of the pre-expectation calculus will need to establish algebraic properties about these mathematical expressions. Our use of distribution axioms(\cref{sec:interpolation}) obviates the need to reason directly about integrals by reducing verification to synthesis.

\paragraph{Martingales} Martingales --- probabilistic analogues of loop invariants --- are used in automated tools to prove termination conditions \citep{Chakarov-martingale,Chatterjee2016,Chatterjee:2016:AAQ:2837614.2837639,Chatterjee:2017:SIP:3009837.3009873,mciver2016new} and properties of expected values \citep{BEFFH16}. Automated martingale synthesis techniques are restricted to linear or polynomial invariants, which alone are unable to prove the accuracy properties we are interested in.

